Sneaky Spikes: Uncovering Stealthy Backdoor Attacks in Spiking Neural Networks with Neuromorphic Data

Deep neural networks (DNNs) have demonstrated remarkable performance across various tasks, including image and speech recognition. However, maximizing the effectiveness of DNNs requires meticulous optimization of numerous hyperparameters and network parameters through training. Moreover, high-performance DNNs entail many parameters, which consume significant energy during training. In order to overcome these challenges, researchers have turned to spiking neural networks (SNNs), which offer enhanced energy efficiency and biologically plausible data processing capabilities, rendering them highly suitable for sensory data tasks, particularly in neuromorphic data. Despite their advantages, SNNs, like DNNs, are susceptible to various threats, including adversarial examples and backdoor attacks. Yet, the field of SNNs still needs to be explored in terms of understanding and countering these attacks. This paper delves into backdoor attacks in SNNs using neuromorphic datasets and diverse triggers. Specifically, we explore backdoor triggers within neuromorphic data that can manipulate their position and color, providing a broader scope of possibilities than conventional triggers in domains like images. We present various attack strategies, achieving an attack success rate of up to 100% while maintaining a negligible impact on clean accuracy. Furthermore, we assess these attacks' stealthiness, revealing that our most potent attacks possess significant stealth capabilities. Lastly, we adapt several state-of-the-art defenses from the image domain, evaluating their efficacy on neuromorphic data and uncovering instances where they fall short, leading to compromised performance.

==> USENIX/rebuttal.tex <==
FINAL:

We thank the reviewers for their valuable comments and suggestions. Due to limited space, we address the primary concerns.

Relevance:
SNNs are used in any operation where DNNs can be because they can handle "regular" data apart from neuromorphic ones, e.g., object recognition or detection. Specific to the latter, SNNs work best for reducing latency and computational costs. Furthermore, in some settings where current DNN-based state-of-the-art methods do not work well, i.e., high-speed scenes of autonomous highway driving, low motion control latency, and low onboard vehicle system power consumption, SNNs could be an alternative.

There are several advantages of neuromorphic data over standard data:
- Energy efficiency: Neuromorphic systems are designed to consume much less power than traditional computing systems, resulting in significant energy savings.
- Real-time processing: Neuromorphic systems can process data in real-time, making them suitable for applications that require fast and accurate responses.
- Robustness: Neuromorphic systems are inherently fault-tolerant and noise resistant. This makes them suitable for applications that require high reliability, such as medical devices.
We emphasize that both SNNs and neuromorphic data have unique challenges. We refer the reviewers to Section 3.2.

Threat model:
Our threat model is different from the adversarial examples one and we want to achieve a backdoor by compromising the training phase of the model and then triggering the backdoor at the test phase. We follow a data poisoning approach compromising the model's integrity, while adversarial examples aim to achieve misclassification at test time. We agree that the attacker would have access to fewer samples depending on the attacker's capabilities. However, we are not poisoning the entire dataset, just a subset defined by $\epsilon$ (we evaluated several options). Additionally, as explained above, we could consider fewer samples.

Sthealthiness:
It is difficult to show neuromorphic data's motion or "dynamism" in a static figure. Thus, we show our attacks in a live demo in the repository provided in the paper. Our dynamic attack can vary its stealthiness by tuning $\gamma$---we show that $\gamma = 0.01$ makes the trigger indistinguishable. Since it is difficult to show the dynamism of the triggers in a figure, we refer the reviewers to check the linked repository where a live demo is available. There the stealthiness of the trigger is better represented---to measure "human detectability," we have conducted a user study. We use SSIM, as previously used in the literature, to measure the triggers' stealthiness. However, we adapt and evaluate it for measuring neuromorphic triggers. Because of computational constraints, we decide to use a small random subset as large as the batch size. We also argue that a random subset would be representative of the whole dataset; thus, the results of using SSIM with the whole dataset are aligned.
We limit our research to digital triggers. The physical triggers require independent research.
Our dynamic attack prioritizes high ASR instead of clean accuracy. The attacker can change the stopping criterion to prioritize a clean high accuracy. We have added experiments showing this.

Defenses:
We have additionally conducted experiments with STRIP (showing its ineffectiveness) and added an adaptive attacker to bypass fine-pruning, who knows the defense applied. Results show that the attack is effective, and we can successfully bypass the countermeasures.

Other:
Q: unclear design of the moving backdoor.
A: Although the previous work authors created the design of the moving backdoor, we briefly explain it here.
The moving backdoor leverages the same trigger as in static backdoors. However, for each time frame, the trigger changes the location, giving a sensation of motion. This trigger aligns more with the neuromorphic data containing no static elements. 

Q: adding triggers to optimal locations in test time?
A: We can add a trigger in an optimal location at test time. An optimal trigger location would depend significantly on the sample itself. However, the dynamic attack does not need a trigger location since it compromises the whole image. We want to thank the reviewer for the interesting observation, and we added the findings to the paper.

We have improved the paper writing and clarified some sections thanks to the reviewers' suggestions, and added new results based on the suggested additional experiments.







Common concern:
We choose the defenses given in the paper since they are some of the most common ones in the literature. Additionally, we have also evaluated our attacks against STRIP. Results show that neuromorphic triggers have more entropy than "standard" triggers, and they are thus not detected. Moreover, we are currently testing the usage of Spectral Signatures [2] for detecting backdoors in SNNs. We have updated the paper accordingly.

Reviewer 1:

Q: Are these algorithms used in practice? If yes, in which applications?
A: SNNs are used in any operation where DNNs are used because they can handle “regular” data apart from neuromorphic ones, e.g., object recognition or detection [1]. Specific to the latter, SNNs work best for reducing latency and computational costs [1]. Furthermore, in some settings where current DNN-based state-of-the-art methods do not work well, i.e., high-speed scenes of autonomous highway driving, low motion control latency, and low onboard vehicle system power consumption, SNNs could be an alternative [2].

Q: What are the advantages of neuromorphic data compared to standard data, and in which applications is this relevant?
A: There are several advantages of neuromorphic data over standard data: 
-	Energy efficiency: Neuromorphic systems are designed to consume much less power than traditional computing systems, resulting in significant energy savings [3].
-	Real-time processing: Neuromorphic systems can process data in real time, making them suitable for applications that require fast and accurate responses [2].
-	Robustness: Neuromorphic systems are inherently fault-tolerant and noise resistant [4]. This makes them suitable for applications that require high reliability, such as medical devices.

Q: I wonder whether the presented attacks are stealthy or not.
A: It is difficult to show neuromorphic data's motion or "dynamism" in a static figure. Thus, we show our attacks in a live demo in the repository provided in the paper. Our dynamic attack can vary its stealthiness by tuning $\gamma$---we show that $\gamma = 0.01$ makes the trigger indistinguishable.

Q: in vision, fixed triggers can be confused by an observer with a postit, for example - is that the case for SNN, too?
A: In that example, the triggers are supposed to be present in a physical scenario. we limit our research to the digital domain. Neuromorphic triggers in the physical domain will require further independent research. Still, triggers in the physical domain could also happen when captured with a DVS camera. We have updated the threat model to clarify that. 

Q: In this context, it would be really helpful if the authors would threat model SNNs a bit better, and explain well which attacks are based on which assumptions, what the attacker's knowledge is, it's goal and give a concrete example where and how an attack could apply in practice.
A: We are updating the introduction section, considering the comments. 

Q: it is not clear to me (a) what the precise argument is here and (b) why defenses other than the two tested should not work on SNN. In general, it would be great if the authors would reason about the choice of the two defenses, as opposed to other mitigations which might(?) work on SNN.
A: We refer to post-training defenses, as ABS, which relies on the “turn points” created by the activation functions. We updated the section to clarify this.
% (b) We choose those defenses since they are some of the most common in the literature. Additionally, we have also evaluated our attacks against STRIP. Results show that neuromorphic triggers have more entropy than "standard" triggers, and they are thus not detected. Moreover, we are currently testing the usage of Spectral Signatures [2] for detecting backdoors in SNNs. We have updated the paper accordingly.

Q: How is human detectability measured here?
A: We have conducted a user study comparing our attacks to measure human detectability. We have updated the paper accordingly.

Q: It would be great if the authors could further provide some numbers about the performance of ABS to verify its bad performance.
A: We provide ABS with T images per class. For example, in the CIFAR10-DVS case, we provide 16 * 10 = 160 images. 
We have added these numbers to the paper.

Q: add an adaptive attack to your fine-pruning evaluation
A: We have implemented an adaptive attacker to bypass fine pruning. Precisely, we include a penalization term in the loss function to ensure that the distance (i.e., MSE) of the backdoor and clean samples in the latent space are close, as done in [5]. We have updated the paper accordingly.

Q: It would still be helpful though to provide a range for this measure, to understand which differences are meaningful for the considered data/setting (as again this data seems to be different to standard vision cases)
A: We will provide additional experiments and discussion to clarify it.

Q: In section 4.1.4., why is ASR maximised instead of high clean accuracy?
A: We wanted to show the upper bound of the performance of the attack. However, the attacker could achieve better clean accuracy by choosing another stopping criterion.

Q: In Figure 6, there are Pruning smart and pruning dynamic. If I understand right, the latter word refers to the attack. It would be great if the authors could clarify this.
A: You are right, and we have updated the paper.

Q: I am not sure what you mean in the related work when writing 'Moreover, they do not detail the core reasoning behind backdoors in SNN'
A: We wanted to emphasize that in previous work, there is insufficient investigation and understanding of how a backdoor applies in the neuromorphic domain. We evaluated the role of stealthiness in the triggers and how it affects the ASR, clean accuracy drop, and defenses, among others.

References:

[1] Rueckauer, B., Lungu, I. A., Hu, Y., Pfeiffer, M., & Liu, S. C. (2017). Conversion of continuous-valued deep networks to efficient event-driven networks for image classification. Frontiers in neuroscience, 11, 682.
[2] Chen, G., Cao, H., Conradt, J., Tang, H., Rohrbein, F., & Knoll, A. (2020). Event-based neuromorphic vision for autonomous driving: A paradigm shift for bio-inspired visual sensing and perception. IEEE Signal Processing Magazine, 37(4), 34-49.
[3] Tavanaei, A., Ghodrati, M., Kheradpisheh, S. R., Masquelier, T., & Maida, A. (2019). Deep learning in spiking neural networks. Neural networks, 111, 47-63. 
[4] Jun Haeng Lee, Tobi Delbruck, and Michael Pfeiffer. Training deep spiking neural networks using backpropagation. Frontiers in neuroscience, 10:508, 2016.
[5] Costales, R., Mao, C., Norwitz, R., Kim, B., & Yang, J. (2020). Live trojan attacks on deep neural networks. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition Workshops (pp. 796-797).

Reviewer 2:

Q: The extension of neural backdoors to SNNs seems relatively straightforward.
A: We want to emphasize that both SNNs and neuromorphic data have unique challenges. In the domain of backdoor attacks, neuromorphic data has limited color possibilities, i.e., 255 in the "regular" domain and two polarities in the neuromorphic domain.

Q: First, I want to encourage the authors to describe that smart backdoors are not sample-specific and are determined across multiple inputs.
A: Indeed, smart backdoors are not sample-specific. However, they could be. We decided to measure the activity area based on the whole dataset to understand the impact of the trigger location and polarity. Precisely, using the whole dataset to determine the most/least active area helps us have a complete experimental setup possible because we consider all the samples. However, measuring the activity area could be done with fewer images, as per batch or even doing it per sample, which will make the attack sample-specific. We have updated the paper to clarify that.

Q: Second, the fact that the entire training dataset is considered for smart backdoors breaks the usual data poisoning assumption
A: We agree that the attacker would have access to fewer samples depending on the attacker's capabilities. However, we are not poisoning the entire dataset, just a subset defined by $\epsilon$ (we evaluated several options). Additionally, as explained above, we could consider fewer samples.

Q: I thus suggest to rephrase the claim on detectability by human analysts as part of the final finding on dynamic backdoors.
A: To be precise about "human detectability," we have conducted a user study. We have updated the paper accordingly.

Q: I want to ask the authors to detail the rationale behind using the SSIM for neuromorphic data and explain why it is average for a random subset.
A: We use SSIM, as it has been previously used in the literature for measuring the stealthiness of the triggers [1], however we adapt and evaluate it for measuring neuromorphic triggers. Because of computational constraints, we decide to use a small random subset as large as the batch size. We also argue that a random subset would be representative of the whole dataset; thus, the results of using SSIM with the whole dataset would be aligned. We have updated the paper to clarify this.

Q: I suggest the authors provide specific (visual) examples for the different triggered inputs to give the reader a better understanding of the differences.
A: As a live demo, we provided visual examples of our different attacks in the linked repository.

% Q: I want to motivate the authors to significantly extend the discussion on backdoor defenses and investigate whether these might apply to SNNs.
% A: This is good suggestion. Based on this and other authors' comments, we have extended the defense section, including more discussion. Additionally, we have also evaluated our attacks against STRIP. Results show that neuromorphic triggers have more entropy than "standard" triggers, and are thus not detected. Additionally, we are currently testing the usage of Spectral Signatures [2] for detecting backdoors in SNNs. We have updated the paper accordingly.

Q: Hence, I suggest the authors rephrase their "finding" on fine-pruning and emphasize its effectiveness.
A: We have updated the paper accordingly.

References:

[1] Liu, Y., Ma, X., Bailey, J., & Lu, F. (2020). Reflection backdoor: A natural backdoor attack on deep neural networks. In Computer Vision–ECCV 2020: 16th European Conference, Glasgow, UK, August 23–28, 2020, Proceedings, Part X 16 (pp. 182-199). Springer International Publishing.
[2] Tran, B., Li, J., & Madry, A. (2018). Spectral signatures in backdoor attacks. Advances in neural information processing systems, 31.

Reviewer 3:

Q: The background section on SNNs should be refined since the concept of SNNs is not clear by just reading this work.
A: We have updated the paper, including more detail on SNNs and overall background improvements.

Q: the concept of polarity needs to be explained better.
A: We have updated the paper to include a clearer explanation.

Q: Algorithm 1 seems to be incorrect, or the second condition in the if statement is redundant.
A: We think the algorithm is correct. We aim to maximize the ASR but ensure the clean accuracy is also good enough. For that, we update the "best" accuracy only if acc $\geq$ acc', or if acc $\geq$ acc' and ASR increases asr $\geq$ asr.' Note that without the terms inside the parenthesis, the clean accuracy could drop to 0 while the ASR goes up, thus making the attack ineffective. We have provided a more detailed explanation in the paper.

Q: The authors should elaborate on if the method is capable of reliably introducing a backdoor with high accuracy (usually > 80\%) even with the knowledge of existing DNN defenses.
A: We want to thank the reviewer for the suggestion. Based on it, we have additionally evaluated the effectiveness of our attack using an adaptive attacker who knows the defense applied. Results show that the attack is effective, and we can successfully bypass the countermeasures. We have updated the paper accordingly.

Q: Additionally, data filtering approaches like [c] should be discussed at least in the related works section to elaborate if the poisoned data could already be filtered out before training.
A: Thanks for the suggestion. Based on this and other authors' comments, we have extended the defense section, including more discussion and results. 
% Additionally, we have also evaluated our attacks against STRIP. Results show that neuromorphic triggers have more entropy than "standard" triggers, and are not detected. We have updated the paper accordingly. Additionally, we are currently testing the usage of Spectral Signatures [1] for detecting backdoors in SNNs. We have updated the paper accordingly.

Q: why the alpha parameter is limited to a range between 0.5 and 0.8?
A: We experimentally saw that values below $\alpha = 0.5$ do not get the backdoor injected, and values above $\alpha = 0.8$ drastically reduce the clean accuracy. Thus, we decided to only show those values for improving readability. We have updated the paper to clarify this.

Q: the paper misses a listing of the computational costs of the approach and no specification of the experimental hardware setting is provided.
A: Thanks for the suggestion. We have redone our experiments and measured the computational costs. The hardware used is a single NVIDIA A100 with 40GB. We have added a table with those results.

Q: Especially, some references should be added. In particular...
A: We have updated the missing references and explanations.

References:

[1] Tran, B., Li, J., & Madry, A. (2018). Spectral signatures in backdoor attacks. Advances in neural information processing systems, 31.

Reviewer 4:

Q: It's difficult to understand why human imperceptibility is important in backdoor attacks.
A: We claim that an imperceptible human trigger could bypass human dataset inspection. This has also been considered in the literature under "human imperceptible" or "stealthy" triggers [1, 2].

Q: If we want to achieve human imperceptible input patterns for causing targeted test-time misclassifications, we already have vast literature on universal adversarial attacks. It does not even require compromising a model.
A: We are aware of adversarial examples that are humanly imperceptible. However, our threat model is different, and we want to achieve a backdoor by compromising the training phase of the model and then triggering the backdoor at the test phase. We want to emphasize that we follow a data poisoning approach which compromises the model's integrity, while adversarial examples aim to achieve misclassification at test time.

Q: I don't think we can construct such patterns in the real world.
A: We limit our research to the digital domain. Neuromorphic triggers in the physical domain will require further independent research. Still, triggers in the physical domain could also happen when captured with a DVS camera. We have updated the threat model to clarify that. 

Q: I am sure this is why many backdoor attacks and defense challenges consider physically realizable patterns as triggers. 
A: Recent work also showed a similar threat model, considering triggers that are not physically realizable, e.g., [1,2].

Q: Most trigger generation approaches, one of this paper's central contributions, have been studied in prior work.
A: Our main contribution, which differs from previous work, is on neuromorphic data and its application in SNNs. As explained in the paper, neuromorphic data has several challenges, which we address in Section 3.2. Additionally, we have improved that section to clarify the challenges.

Q: Do we think we can add a trigger to our optimal locations in the test time?
A: Yes, we can add a trigger in an optimal location at test time. An optimal trigger location would depend significantly on the sample itself. However, the dynamic attack does not need a trigger location since it compromises the whole image. We want to thank the reviewer for the interesting observation, and we added the findings to the paper.

Q: In "Dirty Road Patch Attacks," we can see how we predict the moves of a car and optimize adversarial perturbations for the attack's success, all of which makes the technical contribution of this paper weak.
A: There are several differences between our work and the suggested paper "Dirty Road Patch Attacks." First, the threat model is different. We perform a backdoor attack that compromises the training phase while they perform adversarial examples. Also, we consider the digital domain and the usage of SNNs with neuromorphic datasets. They limit their research to the physical domain and "standard" computer vision systems and datasets. We want to refer the reviewer to Section 3.2 for additional challenges our paper addresses. We have updated the paper to clarify this further.

% Q: only two of them are evaluated against the proposed attacks.
% A: Thanks for the suggestion. Based on this and other authors' comments, we have extended the defense section, including more discussion. We have also evaluated our attacks against STRIP. Results show that neuromorphic triggers have more entropy than "standard" triggers, and they are thus not detected. Additionally, we are currently testing the usage of Spectral Signatures [3] for detecting backdoors in SNNs. We have updated the paper accordingly.

Q: Writing quality is also a problem.
A: Based on the given comments, we have made substantial efforts to improve the writing of the paper.

References:

[1] Nguyen, A., & Tran, A. (2021). Wanet--imperceptible warping-based backdoor attack. arXiv preprint arXiv:2102.10369.
[2] Doan, K., Lao, Y., Zhao, W., & Li, P. (2021). Lira: Learnable, imperceptible and robust backdoor attacks. In Proceedings of the IEEE/CVF International Conference on Computer Vision (pp. 11966-11976).
[3] Tran, B., Li, J., & Madry, A. (2018). Spectral signatures in backdoor attacks. Advances in neural information processing systems, 31.

Reviewer 5:

Q: a more thorough preliminary section would help highlight differences between classical deep neural networks (DNNs) and SNNs.
A: We have updated the preliminary section to include more details.

Q: the novelty of the static and moving backdoor attacks, compared to the existing work (e.g., [1]) should be clarified.
A: Although the design of the static and moving triggers has been addressed in the related work, we emphasize the following differences:
-   We performed a complete experimental setup. Obtaining a deeper understanding of which hyperparameters affect most the performance of the attack.
-   We evaluated the stealthiness of these attacks.
-   We evaluated the viability of these attacks against defense mechanisms.
We have updated the paper to clarify our novelty.

Q: the design of the moving backdoor attack is unclear.
A: Although the previous work authors created the design of the moving backdoor, we briefly explain it here.
The moving backdoor leverages the same trigger as in static backdoors. However, for each time frame, the trigger changes the location, giving a sensation of motion. This trigger aligns more with the neuromorphic data, which contains no static elements. We have updated the paper to clarify this.

Q: some of the results look quite unconvincing, including the ones illustrating the effectives of the new attacks, as it reduces the classification accuracy by 20\% to 50-60\% (on CIFAR).
A: In our experiments, we selected a stopping criterion to achieve the highest ASR possible. However, an attacker could change this to achieve better clean accuracy. We have now evaluated our attack aiming to maintain a high clean accuracy. We have updated the paper accordingly.

Q: Minor comments.
A: We have updated the paper based on the minor comments.

==> USENIX/reviews.tex <==
Review #105A
===========================================================================

Paper summary
-------------
The authors investigate the security of spiking networks against stealthy backdoor attacks. They first outline challenges of spiking networks with regard to backdoors (sequential data, different value range, etc) and then introduce their attacks. They also adapt and evaluate two defences, ABS and fine pruning, on spiking networks.

Detailed comments for authors
-----------------------------
I appreciated reading the paper, as it deals with spiking networks, a method that is not commonly studied in ML security. However, given that this paper has been submitted to a security, not an ML venue, it would have been beneficial to motivate why studying SNN is necessary. Are these algorithms used in practice? If yes, in which applications? 

As a non-SNN expert, I also struggle to understand how the data looks like. What are the advantages of neuromorhpic data compared to standard data, and in which applications is this relevant? As a consequence, I  wonder whether the presented attacks are stealthy or not. For example, consider the moving triggers. It is not clear to me why a moving trigger should be easy to implement in a security setting/in practice, or why it is more stealthy than a fixed trigger (in vision, fixed triggers can be confused by an observer with a postit, for example - is that the case for SNN, too)?
In this context, it would be really helpful if the authors would threat model SNNs a bit better, and explain well which attacks are based on which assumptions, what the attacker's knowledge is, it's goal and give a concrete example where and how an attack could apply in practice.

The authors define several challenges, including that SNN are hard to defend as they 'do not have activation functions which are commonly used in backdoor defenses'. 
Yet, there are also references to papers like Neural Cleanse and STRIP (which both do not rely on specific activation functions), it is not clear to me (a) what the precise argument is here and (b) why defenses other than the two tested should not work on SNN. In general, it would be great if the authors would reason about the choice of the two defenses, as opposed to other mitigations which might(?) work on SNN. 

Finally, there are some claims in the experimental section I struggled to find support for. For example in Section 4.1.4: 'An invisible trigger that cannot be detected by humans can be generated using γ = 0.01'. How is human detectability measured here?
It would be great if the authors could further provide some numbers about the performance of ABS to verify its bad performance, and add an adaptive attack to your fine-pruning evaluation.
Finally, the authors use the well established SSIM measure. It would still be helpful though to provide a range for this measure, to understand which differences are meaningful for the considered data/setting (as again this data seems to be different to standard vision cases).


Further feedback:

[EXPS ONGOING] In section 4.1.4., why is ASR maximised instead of high clean accuracy? This doesn't seem plausible for an attacker that wants the network to be used afterwards.

[DONE] In Figure 6, there are Pruning smart and pruning dynamic. If I understand right, the latter word refers to the attack. It would be great if the authors could clarify this.

[DONE] I am not sure what you mean in the related work when writing 'Moreover, they do not detail the core reasoning behind backdoors in SNN'.

Ethics consideration
--------------------
1. No

Required changes
----------------
- add proper threat modelling
- add detailed description and motivation why SNNs are security relevant
- justify evaluated defenses better
- add adaptive attacks

Reasons to accept the paper
---------------------------
 study backdoor robustness of poorly studied ML algorithm

Reasons to not accept the paper
-------------------------------
- Absence of a threat model
- choice for implanted defenses is not justified
- unsupported claims / methodology in paper

Recommended decision
--------------------
4. Reject

Writing quality
---------------
2. Well-written

Confidence in recommended decision
----------------------------------
2. Fairly confident


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #105B
===========================================================================

Paper summary
-------------
The paper describes backdooring attacks against spiking neural networks (SNNs). In contrast to deep neural networks, SNNs are more energy efficient and involve a temporal component in processing input, represented by "neuromorphic data." The latter adds a new dimension to backdooring such models, extending static triggers to triggers that are dynamic across time. The authors exercise different trigger types and show their effectiveness based on three (neuromorphic) datasets. Additionally, the evaluation inspects defenses against backdooring attacks and how these can be extended to SNNs and analyzes the attacks' stealthiness.

Detailed comments for authors
-----------------------------
Spiking neural networks (SNNs) have experienced a revival recently. Combined with backdooring attacks that have also received much attention in the past couple of years, the paper works on a particularly timely combination. I have found myself reading the paper with great interest. However, backdoors of SNNs are somewhat "derivative" from a scientific point of view, impacting novelty, even though there does not exist a paper on this topic yet. The extension of neural backdoors to SNNs seems relatively straightforward. In this regard, it is challenging to give actionable advice. In the following, however, I detail a few more aspects in three categories (Method description, stealthiness, and defenses) in the hope of helping improve the paper further:

#### Method description

[DONE]- **Smart backdoors.** In Section 3.5, it does not become clear that smart backdoors are actually averaged across multiple input samples. Only in Section 4.1.3, the authors state that *"the activity sum is done over all the images in the training set."* First, I want to encourage the authors to **describe that smart backdoors are not sample-specific and are determined across multiple inputs.** Second, the fact that the entire training dataset is considered for smart backdoors breaks the usual data poisoning assumption.

#### Stealthiness

- **Human visibility/detectability.** In Section 4.1.4, the authors find that *"an invisible trigger that cannot be detected by humans can be generated using $\gamma=0.01$."* For making such a strong statement, the evaluation requires conducting a user study to verify what triggers humans perceive and what they do not. I thus suggest to **rephrase the claim on detectability by human analysts as part of the final finding on dynamic backdoors.**

[DONE] - **Structural similarity index measure (SSIM).** While the SSIM can be a better alternative to the mean-squared error (MSE) for image data, the authors fail to argue why this applies to neuromorphic data. Moreover, the authors specify to *"average over 16 randomly selected images from the test set"* without detailing why they limited the number to 16 instances. I want to ask the authors to **detail the rationale behind using the SSIM for neuromorphic data and explain why it is average for a random subset.** Moreover, the specified ratios (for instance, in the introduction as part of the list of contributions) are difficult to interpret: *"[...] our dynamic trigger achieves the best stealthiness, up to 99.9 SSIM, while other methods, like static or moving triggers, achieve 98.5.% SSIM."* Judging by these numbers, there is no practical difference. I suggest the authors **provide specific (visual) examples for the different triggered inputs to give the reader a better understanding of the differences.**

#### Defenses

- **Shallow discussion of defenses.** While I appreciate the authors' effort to look at defenses, the extent is limited. In particular, the authors discuss two approaches: ABS (Liu et al., CCS 2019), which is not applicable according to the authors, and Fine-Pruning (Liu et al., RAID 2018), an early approach that even works rather well in this case. However, a large portion of defenses in the field is not discussed at all. Hence, I want to motivate the authors to **significantly extend the discussion on backdoor defenses** and investigate whether these might apply to SNNs.

- **Effectiveness of fine-pruning.** According to the results the authors present in Section 4.2.2, fine-pruning is effective against the proposed backdooring attack against SNNs. In light of this, the second sentence of the presented finding *"Still, this depends on the dataset characteristic and the trigger type,"* seem unjustifiably negative. Except for the moving trigger, where the ASR is reduced from 100% to 90%, the decrease in ASR is distinctive. Hence, I suggest the authors **rephrase their "finding" on fine-pruning and emphasize its effectiveness.**

Ethics consideration
--------------------
1. No

Reasons to accept the paper
---------------------------
+ **Attacks against a timely line of research.** With spiking neural networks (SNNs), the authors have chosen a topic of machine learning research that has recently been revived. Discussing attacks and defense in this scope is interesting.

+ **Well-written and easy to follow.** The paper is well-structured, the descriptions are clear and easy to follow, and the depiction and plots assist the understanding of the paper well. All this makes the paper accessible to the unfamiliar reader.

+ **Consideration of different facets of the problem.** The authors cover many different aspects of neural backdoors against SNNs. While a few aspects can be extended, the paper makes a sound impression overall.

Reasons to not accept the paper
-------------------------------
- **Novelty.** While neural backdoors for spiking neural networks have not been discussed in the literature, the paper exercises the known concept for a new application. As such, the novel scientific insight is small.

- **Interpretation of the SSIM.** The authors use SSIM over MSE but do not discuss why SSIM might be preferable for neuromorphic data. Moreover, when discussing specific values of this similarity measure, specific visual examples would help grasp the actual difference behind the reported numbers.

- **Shallow discussion of defenses.** Additionally discussing defense is a great effort. However, as the authors pick two examples out of a plethora of defensive mechanisms against neural backdoors, the overall discussion is limited.

Recommended decision
--------------------
2. Accept on Shepherd Approval

Writing quality
---------------
3. Adequate

Confidence in recommended decision
----------------------------------
2. Fairly confident


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #105C
===========================================================================

Paper summary
-------------
In this paper, the authors examine four different trigger methods for conducting a targeted poisoning attack on Spiking Neuronal Networks (SNNs), two of them being newly developed in this work. This is a novel research area with few related works. Previous works introduced the basic proof of the feasibility of targeted poisoning attacks on SNNs with two of the analyzed triggers or focused on poisoning attacks on classical neuronal networks. The approaches are evaluated on different classification tasks in the image domain and the properties and quality of the introduced backdoor are measured.

Detailed comments for authors
-----------------------------
This is a well-written paper on a timely topic and one of the first works in the area of poisoning Spiking Neuronal Networks (SNNs). The work elaborates on four different backdoor triggers showing the influence factors an adversary must consider when conducting an attack. In previous works, only the general proof of applicability was provided with basic trigger mechanisms. The core contribution of the authors is a sophisticated trigger method and the analysis of influence factors.

This work contains a clear motivation section and a valid threat model.  The open-sourced code will greatly benefit future research in the field of security of SNNs, as it enables the replication of results and facilitates progress in this area. 

Albeit the paper depicts a promising approach and delivers interesting insights, some sections contain weaknesses and need to be addressed by the authors. Especially, the background section on SNNs should be refined since the concept of SNNs is not clear by just reading this work. The authors force the reader to consult additional literature to comprehend the presented approach. First and foremost, the concept of polarity needs to be explained better. The statements about “several frames per data point” and “four different values” at the beginning of C1 and C2 only got clear after reading external material, which should be addressed by the authors. The authors can align to the explanation of [1] combined with Figure 1 of this paper or of [1] respectively. Further, Section 4 introduces how neuromorphic data can be generated, which should also be mentioned early in the paper. Additionally, a visualization similar (perhaps a bit simpler) to Figure 2 in [27] should be included in this paper. If the authors need more space, one could leave out the second set of equations in Section 3.5, which did not bring additional benefit. In addition, adjustments in the background section, Section 4.2.1 should also be made to clearly explain the procedure, since in the current version it was necessary to read them several times. 

Moreover, some experimental outcomes need to be revisited. The results of Figure 10-12 are poorly commented, since the scale in the Figure is -5 and not 10% as mentioned by the authors and somehow the clean accuracy also increases in between, which is not discussed in Section 4.1.1. Further, the authors claim for Figure 16-19 a maximum of 4% degradation. However, Figure 19 seems to show more than 4%. In addition to these ambiguities, Algorithm 1 seems to be incorrect, or the second condition in the if statement is redundant.

Based on the results, especially Figure 6, one can conclude that poisoning attacks on SNNs bring no danger to real-world systems when they are equipped with a basic defense like [31]. The authors should elaborate on if the method is capable of reliably introducing a backdoor with high accuracy (usually > 80%) even with the knowledge of existing DNN defenses. Since only two defenses (from year 2018 and 2019) have been evaluated, it is questionable if there are other, newer technologies out there that remove the backdoor in all cases, which should be discussed and evaluated more deeply. It would be sensible to evaluate an adaption of [7] and consider [b] as newer work. Additionally, data filtering approaches like [c] should be discussed at least in the related works section to elaborate if the poisoned data could already be filtered out before training.

Within the experiment section, it remains unclear to the reader, why the alpha parameter is limited to a range between 0.5 and 0.8. The equation itself reminds of the constraint method from Bagdasaryan et. al [a] in the domain of federated learning. In related backdoor papers, an alpha range between 0.1 and 0.9 is tested, which should also be done within this work. Besides, the paper misses a listing of the computational costs of the approach and no specification of the experimental hardware setting is provided.
The paper also contains a few contextual and editorial weaknesses that need to be fixed or improved. Especially, some references should be added. In particular: 

-	Add a reference to the following sentence: “For example, the computer vision domain has achieved top performance in autonomous driving.”

[DONE] -	Add a reference to the following statement: “In the image domain, the trigger can be a pixel pattern in a specific part of the image.”
[DONE]-	D_bk is already used in Section 2.1, but not introduced beforehand or directly after the usage. We found some explanation later in Section 3.3, which should be shifted to the first occurrence. Further, the authors should clearly state what bk stands for (k for trigger is not intuitive, for b it is not clear as well, but one could assume “backdoor”).
[DONE]-	The following sentence should contain a reference for MLPs to ease the access to further resources for the reader: “To explain the differences between DNNs and SNNs, let us consider an example with a multilayer perceptron (MLP), which consists of layers containing neurons.” The same holds for ReLU within the same section.
[DONE]-	An explanation or a reference should be given for the following statement: “The explained architecture is linear, making it difficult to train.”
[DONE]-	Provide some references for further research after the following sentence: “An advantage of DVS cameras is that they provide an almost instantaneous representation of the visual scene in a very compressed form, which facilitates posterior data processing.”
[DONE]-	Provide references for Google Cloud and AWS in Section 3.1.
[DONE]-	The following sentence also needs a reference as evidence: “For example, autoencoders are used for denoising tasks, where we would usually require clean (denoised) and noisy versions of the image to train the autoencoder, i.e., the autoencoder is trained on image pairs.”
[DONE]-	The term “l_p-ball” in Section 3.5 is confusing. Either supplement it with a footnote or explain the concept without the term.
[DONE]-	Add a reference to ATIS sensors in Section 4.
[DONE]-	For Figure 5, the red lines should also be mentioned in the legend as accuracies from Table 1. This prevents confusion by the reader when analyzing the graphics.

In summary, the authors introduce a novel method to embed a backdoor into an SNN, which is a timely topic, and evaluate the feasibility and influence factors by conducting an experimental study showing promising results. However, the paper is not self-contained and shows editorial weaknesses. Further, some experiments should be added to the evaluation and discussion and a final statement about the risk in real-world scenarios under the most recent defense techniques should be added. These changes could be done under a minor revision.


References:
[a] E. Bagdasaryan, A. Veit, Y. Hua, D. Estrin, and V. Shmatikov, “How to backdoor federated learning,” in International Conference on Artificial Intelligence and Statistics, 2020, pp. 2938–2948.
[b] D. Wu and Y. Wang, “Adversarial neuron pruning purifies backdoored deep models,” Advances in Neural Information Processing Systems, vol. 34, pp. 16913–16925, 2021.
[c] Y. Li, X. Lyu, N. Koren, L. Lyu, B. Li, and X. Ma, “Anti-backdoor learning: Training clean models on poisoned data,” Advances in Neural Information Processing Systems, vol. 34, pp. 14900–14912, 2021.

Ethics consideration
--------------------
1. No

Required changes
----------------
-	Refine the background section to make the paper self-contained. Especially, focus on the explanation of polarity.
-	Clarify the confusion regarding the results and the algorithm mentioned above.
-	Add experiments for the full value range of the alpha parameter.
-	Discuss data cleaning approaches in the related works section.
-	Resolve the editorial weaknesses listed in the comments section of this review.

Reasons to accept the paper
---------------------------
-	Timely and interesting topic in an unexplored research area
-	Well-written paper
-	Clear motivation and threat model
-	Helpful results to facilitate future research in the respective area
-	Reproducible results due to open-sourced code

Reasons to not accept the paper
-------------------------------
-	Weak background section
-	Editorial weaknesses
-	Open questions regarding the results
-	No significant evidence of a threat for a system leveraging recent defenses
-	No evaluation of the computational costs and no information about experimental settings
-	Missing experiments for certain parameters

Recommended decision
--------------------
2. Accept on Shepherd Approval

Writing quality
---------------
2. Well-written

Confidence in recommended decision
----------------------------------
3. Highly confident (would try to convince others)


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #105D
===========================================================================

Paper summary
-------------
This paper studies the vulnerability of spiking neural networks to backdoor attacks. Specifically, the paper explores the human-imperceptible trigger patterns designed for backdooring spiking neural networks. As neuromorphic datasets encode movements of an object over multiple frames, the paper presents smart and dynamic backdoor attacks that place a backdoor trigger at the optimal spots and/or move the trigger along with an object's movement. In evaluation across three neuromorphic tasks, the paper shows a high backdoor success with a minimum accuracy drop. The paper shows that existing defenses (ABS and fine-pruning) are ineffective against the proposed backdoor attacks. The paper also measures the human imperceptibility of constructed triggers with pixel-level distances and concludes by suggesting future work.

Detailed comments for authors
-----------------------------
I have two major concerns about this paper.


(1) It's difficult to understand why human imperceptibility is important in backdoor attacks. I've seen many prior works on backdoor attacks pursuing human imperceptibility, but I suspect this is from the confusion about the threat model.

If we want to achieve human imperceptible input patterns for causing targeted test-time misclassifications, we already have vast literature on universal adversarial attacks. It does not even require compromising a model. The adversary can offer a clean model to the victim, while the attacker crafts many universal adversarial patterns for multiple classes. They can use them when they want.

It also contradicts the practical attack claims. Suppose we have human imperceptible triggers, as shown in Figure 3. I don't think we can construct such patterns in the real world. I am sure this is why many backdoor attacks and defense challenges consider physically realizable patterns as triggers. It makes much sense that the human-imperceptibility should be achieved by an object that can be nicely blended into a scene, such as a sticky note attached to a stop sign (Gu et al.).


(2) Most trigger generation approaches, one of this paper's central contributions, have been studied in prior work. 

In the universal adversarial attacks, adversarial patch attacks, and/or backdoor attacks, we can find similar spacial optimization techniques that search the best locations for a trigger. (I am also skeptical about this assumption, too. Do we think we can add a trigger to our optimal locations in the test time?) 

Regarding the dynamic backdoors, we can search with the keyword "backdoor attacks against video datasets" and find many techniques. In addition, in a recent paper at the same conference, "Dirty Road Patch Attacks," we can see how we predict the moves of a car and optimize adversarial perturbations for the attack's success, all of which makes the technical contribution of this paper weak.


I have some more comments about two minor things.

(1) The problem this paper pointed out is "the attacks and counter-measures for SNNs have been almost fully unexplored." The paper answers the attacks part, but there is no full exploration of the defense side. Moreover, the paper's contribution is "We observe that existing (adapted) defenses can be ineffective against backdoor attacks in SNNs." But in Sec 6.3, the paper criticizes existing defenses without an evaluation; only two of them are evaluated against the proposed attacks.

(2) Writing quality is also a problem. 

1. Figure 1 does not show how neuromorphic data is composed of frames and polarities.
2. More details regarding the training of spiking neural networks may be required; the only information is in the evaluation section, mentioning that the paper uses the 'spiking jelly framework.'
3. It's difficult to understand this: "SNNs do not work with continuously changing time values (like DNNs) but operate with discrete events that occur at certain points in time." What does it mean by "like DNNs"?

Ethics consideration
--------------------
1. No

Comments for ethics consideration
---------------------------------
No ethics concern

Required changes
----------------
1. Clarify why "human-imperceptibility" is important in backdoor attacks.
2. Clarify the technical novelty of the proposed methods over the techniques prior work uses.
3. Run evaluation with existing defenses the paper criticizes.
4. Improve the writing quality.

Reasons to accept the paper
---------------------------
1. The paper studies the backdoor vulnerability of spiking neural networks.
2. The paper studies techniques to construct human-imperceptible triggers to achieve the goal.
3. The paper tests a few existing defenses against backdoor attacks.

Reasons to not accept the paper
-------------------------------
1. If the human imperceptibility of triggers is the goal, we can achieve this through adversarial attacks.
2. I am oncerned about the novelty. Many similar attack approaches have been explored in prior work.
3. In Sec 6.3, the paper claims the ineffectiveness of existing defenses without any evaluation (overclaims).
4. Poor writing quality (more detailed comments above).

Overall, I am not sure a revision in a short period can address all the concerns.

Recommended decision
--------------------
4. Reject

Writing quality
---------------
4. Needs improvement

Confidence in recommended decision
----------------------------------
3. Highly confident (would try to convince others)


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #105E
===========================================================================

Paper summary
-------------
The paper considers the design and analysis of backdoor attacks on spiking neural networks. The authors improve and evaluate static and moving backdoor attacks, as well as introduce new smart and dynamic backdoor attacks. Performance, in terms of accuracy on clean data sets and attack success rate (ASR) on the backdoor data are evaluated on three sniping datasets.

Detailed comments for authors
-----------------------------
While the paper considers an interesting topic, it is unclear what the novel contributions are compared to the state of the art. In particular, there are several paper limitations that should be addressed.

-- for readers with limited background in spiking neural networks (SNNs), it is hard to follow parts of the paper highlighting the SNN training and security challenges. a more thorough preliminary section would help highlight differences between classical deep neural networks (DNNs) and SNNs; e.g. the notion of polarity, as it is critical to understand  for instance what is a polarity e.g. p_3 of a mask used to define attacks in 3.5; or e.g., why is the approach from 3.6 (dynamic backdoor attack) specific for SNNs, as it seems quite DNN-like.

- the novelty of the static and moving backdoor attacks, compared to the existing work (e.g., [1]) should be clarified. Also, the design of the moving backdoor attack is unclear -- from the problem formulation, it seems that the attacks focus on models used for single image classification; if that's the case, it is unclear how is then the problem mapped into classification of time-series/sequence of images (i.e. over a frame T)

- some of the results look quite unconvincing, including the ones illustrating the effectives of the new attacks (which is the main contribution of the paper). For example, the results in Fig. 5 show that the dynamic backdoor attack does not perform well on DVS128 and CIFAR10-DVS datasets (i.e. 2 out of 3 considered datasets), as it reduces the classification accuracy by 20% to 50-60% (on CIFAR). Similarly, for smart attacks on some of the datasets. 

Minor comments: 
[DONE] - n is used both for the size of the clean dataset as well as the number of lines in the smart backdoor attack.
- some of the "Findings" have limited support in the text. for example, in Section 4.1.4 that "an invisible trigger cannot be detected by human"... as there have been no human experiments; even the stealthiness analysis have not been presented up to that point

Ethics consideration
--------------------
1. No

Required changes
----------------
- SNN preliminaries
- showing effectiveness of the attacks introduced in the paper

Reasons to accept the paper
---------------------------
- the paper considers an interesting problem

Reasons to not accept the paper
-------------------------------
- it is unclear how effective the proposed attacks are

Recommended decision
--------------------
4. Reject

Writing quality
---------------
3. Adequate

Confidence in recommended decision
----------------------------------
2. Fairly confident



==> sections/01-old_intro.tex <==
\section{Introduction}

Deep neural networks (DNNs) have achieved high performance in numerous machine learning tasks in different domains, like computer vision~\cite{krizhevsky2012imagenet}, speech recognition~\cite{graves2013speech}, or text generation~\cite{brown2020language}. The fast-evolving domain of deep learning (DL) has pushed the research domain to develop more complex and capable algorithms~\cite{szegedy2015going}.

One key aspect of DNNs that has contributed to their success is their ability to learn from large amounts of data and discover complex patterns.
This is achieved through multiple layers of interconnected neurons. %, which process the input data and pass it through the network\onote{what do you mean by the last part?}. 
The connections between these nodes are weighted, and the weights are adjusted during training to minimize error and improve the accuracy of the model.
DNNs have a large number of hyperparameters that can be tuned to achieve optimal performance on a given task. These hyperparameters include the number of layers and neurons in the network, the learning rate (LR), the activation function used, and the optimization algorithm employed. Careful optimization of these hyperparameters is crucial for achieving good performance with DNNs.\onote{Same comment in abstract, is it still efficient to use SNNs for different hyperparameters? if so, then ignore my comment}

One of the main challenges in training DNNs is the need for large amounts of labeled data, which can be expensive and time-consuming to obtain and can also be a limiting factor in developing DNNs for certain tasks. To address this issue, researchers have explored techniques such as transfer learning, which allows a pre-trained model to be fine-tuned for a new task using a smaller amount of data, and unsupervised learning, which allows models to learn from unlabeled data~\cite{torrey2010transfer}.\onote{Why do we have this paragraph? we do not use or need transfer learning}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/samples.pdf}
    \caption{Normal and neuromorphic data samples.\onote{it is a long figure for an example}}
    \label{fig:sample}
\end{figure}

Overall, DNNs have had a significant impact on machine learning and have the potential to revolutionize a wide range of applications. \onote{I think we spent a lot of space for DNNs so far}
However, the increasing complexity and computational requirements of these models have led researchers to explore alternative approaches, such as spiking neural networks (SNNs)%, to address these challenges
~\cite{ghosh2009spiking, tavanaei2019deep}. \onote{Why do we have the following sentence? it also breaks the flow}Despite these limitations, the continued development and improvement of DNNs and other DL techniques is an active area of research that holds great promise for advancing the field and enabling the development of even more powerful and capable machine learning algorithms.

\onote{Isn't this paragraph repeating the previous one (with different references)? Why do we describe as a new challenge?}Another challenge to overcome is the electricity consumption, directly related to the training time and the complexity of the models~\cite{dhar2020carbon}. Therefore, since the trend is to train more complex algorithms, the costs of training such models increase exponentially; as a solution SNNs was introduced, which enables energy-efficient training of DNNs, achieving similar performance as the standard networks~\cite{eshraghian2021training, fang2021incorporating}.

SNNs have the potential to significantly reduce the energy consumption of neural networks, being up to $12.2 \times$ better energy efficient, making them more practical for real-world applications~\cite{kundu2021spike}. In addition to their energy efficiency, SNNs have several other benefits. For example, they can process data in a more biologically plausible manner, such as neuromorphic data (see~\autoref{fig:sample}), which makes them well-suited for tasks that involve sensory data processing. SNNs can also be more robust to noise and perturbations, making them more reliable in real-world situations~\cite{lee2016training}.
\onote{Maybe explain the left most column of the figure, saying each data sample is a GIF, and they are hand gestures}

Despite these advantages, SNNs also have some limitations. For example, they are often more challenging to train than standard DNNs and may require more data to achieve good performance~\cite{tavanaei2019deep}. In addition, SNNs are still a relatively new and emerging technology, and more research is needed to understand their capabilities and limitations fully. \onote{Do we need to mention the limitations of SNNs? it is not much related to our work, and it breaks the transition}

Overall, the development and use of SNNs is an active area of research that holds great promise for addressing some of the challenges associated with DNNs and enabling the development of more energy-efficient and biologically plausible machine learning algorithms.\onote{I think we do not need this paragraph}

Neural networks are generally subject to privacy and security attacks, e.g., adversarial examples~\cite{szegedy2013intriguing}, inference~\cite{carlini2021extracting}, model stealing~\cite{jagielski2020high}, and backdoor attacks~\cite{gu2019badnets}. Backdoor attacks are a case of threat where malicious samples containing a trigger are included in the dataset at training time. After training, a backdoor model correctly performs the main task at test time while achieving misclassification when the input contains the trigger. 
\onote{mention the countermeasures as well. Then say that these attacks and countermeasures are well investigated for DNNs, yet SNNs are not well explored.
 because of their different structure and dataset, it is an interesting problem. 
 Here mention your poster paper, and its limitations like only considering static trigger, not stealthy and no defense etc.}
In this paper, we investigate the viability of backdoor attacks in SNNs, providing different procedures for injecting the backdoor, from already known techniques in DNNs to SNNs and neuromorphic data-specific triggers.
\onote{mention we also modify the countermeasures for it}


\subsection{Our Contributions}\onote{no need to subsection if there is only one}

Our contributions can be summarized in the following:

\begin{itemize}
    \item To the best of our knowledge, we have investigated the first backdoor attack in SNNs using neuromorphic data. \onote{we are not the first, what about your poster?}
    \item We have explored different backdoor injecting methods, which achieve up to 100\% accuracy in both main and backdoor tasks. We have even developed a dynamic backdoor attack, which is invisible to human inspection. \onote{Stealthiness is important we should emphasize it}
    \item We have adapted a state-of-the-art countermeasure from DL to SNNs, and proposed insights as a possible defense mechanism to be adopted. 
    \item We share our code to allow the reproducibility of our results along with easing future security analysis of SNNs\footnote{https://anonymous.4open.science/r/Backdoor-attacks-in-SNN/}.
    \onote{As we discussed before, can you put some gifs with triggers in the repository? Here you can mention them as well}
\end{itemize}

==> sections/rebuttal.tex <==
Dear Reviewers,

We appreciate your valuable feedback. Due to space constraints, we provide a concise list of changes made concerning Reviews 1 and 2, and we:

1.	Added additional references in the introduction and clarified the explanation of static and moving triggers.
3.	Merged contributions three and four for clarity.
4.	In Section III: clarified the definition of the S masks, removed the formula for p' and included additional explanation, omitted the last two formulas in Section E, rephrased confusing sentences and improved the overall explanation, and reformatted Section F formulas for readability.
5.	Clarified "spiking AE."
6.	Explained the difference in usage of the "Default Training Settings" and STDP/Adam.
7.	Reported average results in the text to improve readability.
8.	Added additional details for neuromorphic data.
9.	Added DNN vs. SNN comparisons.
10.	Changed the color of the STRIP figures.
11.	Run the experiments that confirm the hypothesis of the "adaptive attacker." 
12.	Expanded related work.
13.	Clarified neuromorphic vs. video backdoors.
14.	Improved CIFAR-10 dynamic backdoor results explanations.

Reviewer 3. 
We are working on clarifying the following concerns on the paper. Due to space limitations, we provide a summary:

1.	"Stealthiness of dynamic backdoor attack." 
We adjusted our claim and stated that we introduced the first dynamic backdoor attack on the neuromorphic dataset, which is highly stealthy, particularly at γ=0.01, where only 4\% of the participants found the trigger.

2.	"Ensuring smooth trigger changes." 
The trigger's smooth changes are achieved by randomly moving it to nearby locations (giving a sense of smoothness), making it difficult to detect compared to static triggers.

3.	"Location of the moving trigger." 
Triggers' location and polarity influence the attack's performance of the static triggers. A static trigger located in an area with the same polarity as the trigger will "merge," making the trigger not work. Moving triggers can surpass this because of the location change. This was introduced in previous work [1].

4.	"Smart trigger optimization." 
The selection of the optimal mask is not done manually, and the polarity is determined based on the characteristics of the most/least active area.

5.	"Measuring the most active input area." 
To measure the activity of an area, we count the changes in polarity from one polarity to another. Since p0 represents no movement, we do not consider that as "activity." For example, the change from p2 to p1 or p0 to p1 is counted as 1. In contrast, the change from p2 to p0 does not count due to the representation of a "movement" state to a "no movement" state.

6.	"Formula for the most active mask." 
We removed the equation and explained it in the text for improved clarity.

7.	"Computation of perturbation using AE."
The difference with adversarial examples is that AE is trained simultaneously with the model. This is impossible in adversarial examples due to the threat model, which does not allow tampering with the training phase. Here, AE is tailored explicitly for the dataset and the model.

8.	"Placement of main evaluation results." 
We will integrate the main evaluation results in the main body of the paper.

9.	"Clarification on smart trigger design." 
A smart trigger's design is to determine what affects the trigger's success. We found that the attack's success regarding the trigger polarity is linked to the background polarity. That is why we evaluate the area's least and most common polarities. 

10.	"Confusing statements regarding moving triggers." 
We are improving the explanation of the moving trigger's behavior compared to static triggers. Unlike moving triggers, smart triggers leverage "contrast" between the background and the trigger. In the moving triggers, we refer to the same trigger polarity as the background. We will clarify the behavior of moving triggers compared to static triggers and distinguish them from smart triggers in terms of polarity.

11.	"Separate experiments for α and γ." 
Our experiments were performed for independent α and γ values, experimenting on all combinations (see Figure 4). We will improve the explanation to provide a more comprehensive understanding of the dynamic attack's performance on different datasets.

Additionally, we corrected the color representation of ASR lines in Figure 4, and we will improve the overall coherence and readability of the paper.

==> sections/shepherd.tex <==
R1: For the moving trigger: Formulate mathematically how the trigger k smoothly changes from frame to frame, creating a moving effect and optimally decide on which input “activity area”, the trigger should be placed.

We updated Section II.D to include a mathematical formulation of the moving trigger:

To create a moving trigger, a binary mask $m$ is created to cover $\mathbf{x}$. $m$ is created based on the trigger location and size. In moving riggers, the trigger moves so $m$ is updated per frame $m_{t+1} = m_t >> 2$ by shifting 2 pixels to the right. Then, the mask merges with the trigger $\hat{\mathbf{x}}_t = \mathbf{x}_t \oplus m_t$, and the chosen polarity is set in the given area.

R2: For the dynamic trigger also, same requirement, as in R1. Please provide a more mathematically sound design of the dynamic trigger.

This is already in the paper.

R3: Give a detailed description and intuition of why polarity "p" is and is used to determine the most active mask.

We clarified it in Section III.E.

R4: Consider more datasets for the experimental evaluation.

[ONGOING] Should I dont more experiments? in another dataset?
